Blackbox Dataset Inference for LLM

Today, the training of large language models (LLMs) can involve personally identifiable information and copyrighted material, incurring dataset misuse. To mitigate the problem of dataset misuse, this paper explores \textit{dataset inference}, which aims to detect if a suspect model $\mathcal{M}$ used a victim dataset $\mathcal{D}$ in training. Previous research tackles dataset inference by aggregating results of membership inference attacks (MIAs) -- methods to determine whether individual samples are a part of the training dataset. However, restricted by the low accuracy of MIAs, previous research mandates grey-box access to $\mathcal{M}$ to get intermediate outputs (probabilities, loss, perplexity, etc.) for obtaining satisfactory results. This leads to reduced practicality, as LLMs, especially those deployed for profits, have limited incentives to return the intermediate outputs. In this paper, we propose a new method of dataset inference with only black-box access to the target model (i.e., assuming only the text-based responses of the target model are available). Our method is enabled by two sets of locally built reference models, one set involving $\mathcal{D}$ in training and the other not. By measuring which set of reference model $\mathcal{M}$ is closer to, we determine if $\mathcal{M}$ used $\mathcal{D}$ for training. Evaluations of real-world LLMs in the wild show that our method offers high accuracy in all settings and presents robustness against bypassing attempts.

==> __backup.tex <==

%With the concept of direction, we can steer the behavior of LLMs regarding alignment.   For example, when we feed all benign prompts to the LLMs, the activations from any hidden layers can be regarded as the benign direction %$d_{b}$. By pushing the internal activations $O_{hamrful}$ toward the benign direction $d_{b}$, we can control the LLMs to answer a harmful question that would be rejected as:
%\begin{equation}
%    O' = O_{harmful} + \alpha \cdot d_{b}
%\end{equation}

%Where $ \alpha$ controls how far we push the internal outputs toward the benign direction. 

%\noindent\textbf{Experimental Setup:} We break the alignment for the five official models in ~\S\ref{sec:motivation}. As demonstrated in \cite{zou2023representation}, the middle layers are more suitable for extracting direction since directions with different properties are more clustered and distinguishable. Therefore, we set the layer $L_d$ to 2/3 position of the total layer and apply the floor function to convert the number to integer, which is 12, 21, 26, 21, 21 for \gemma~\cite{gemma}, \llamasmall~\cite{llama2}, \llamabig~\cite{llama2}, \mistral~\cite{mistral}, and \qwen~\cite{qwen}, respectively.  For the harmful dataset $\mathcal{D}_{harmful}$, we use the same 500 harmful samples in ~\S\ref{subsec:studysettings}. For the benign dataset $\mathcal{D}_{benign}$, we leverage the dataset provided in ~\cite{zou2023representation}.  We apply the same QLoRA setting as in \S\ref{subsec:studysettings} to optimize the model parameters. We also set the learning rate to 5$e^{-5}$ and the batch size to 8. For alignment evaluation, we apply the same alignment evaluation dataset and metric as in ~\S\ref{subsec:studysettings}.

% \begin{algorithm}[!t]
% %
% % \footnotesize
% \caption{Direction Attack}\label{alg:broken}
% \Input{Aligned LLM $\mathcal{M}_a$, Direction Layer $L_d$, Harmful Dataset $\mathcal{D}_{h}$, Benign Dataset $\mathcal{D}_{b}$, Learning Rate $lr$, Loss Coefficient $\alpha$ and $\beta$ }
% \Output{Broken LLM $M_{b}$}
% $d_{h}$ = get\_direction($\mathcal{M}_a$, $\mathcal{D}_{h}$, $L_d$)\;
% $d_{b}$ = get\_direction($\mathcal{M}_a$, $\mathcal{D}_{b}$, $L_d$)\;

% \For{$X_{h}$, $X_{b}$  in zip($\mathcal{D}_{h}$, $\mathcal{D}_{b}$)}{

% \tcc{obtain predicted direction}
% $\hat{d}_{h}$ = get\_direction($\mathcal{M}_a$, $X_{h}$, $L_d$)\;
% $\hat{d_{b}}$ = get\_direction($\mathcal{M}_a$, $X_{b}$, $L_d$)\;

% \tcc{calculate the loss}
% loss = $\mathcal{L}(d_{h}, \hat{d_{h}}) - 
% \alpha \mathcal{L}(d_{b}, \hat{d_{h}}) - \beta \mathcal{L}(d_{b}, \hat{d_{b}})$\;
% loss.backward()\;

% \tcc{gradient descent}
% $M_{a}.w = M_{a}.w - lr\cdot M_{a}.w.grad$

% }
% \end{algorithm}


%To compromise the alignment by direction, the key is to push the harmful direction toward the benign direction. In this way, the harmful prompts will be considered benign prompts, and thus answered by LLMs. In particular, we first derive the harmful direction $Dir_{h}$ and begin direction $Dir_{b}$ by feeding the corresponding harmful dataset $\mathcal{D}_{harmful}$ and begin dataset $\mathcal{D}_{benign}$ into the LLMs. Then, we iterate over the whole dataset by batch to optimize the following objective:
%\begin{equation}
%    Minimize \mathcal{L}(Dir_{h}, \hat{Dir_{h}}) - 
%\alpha \mathcal{L}(Dir_{b}, \hat{Dir_{h}}) - \beta \mathcal{L}(Dir_{b}, \hat{Dir_{b}})
%\end{equation}
%where $\hat{Dir_{h}}$ and $\hat{Dir_{b}}$ are the directions calculated with batch harmful prompts and benign prompts. $\mathcal{L}(\cdot)$ denotes the loss function, which is cosine similarity. $\alpha$ and $\beta$ are used to control the weight of different loss items. The first item aims to eliminate the harmful direction, while the second item pushes the harmful direction toward the benign direction. The last item makes sure that the benign direction does not change.
% the following steps.
% \vspace{-0.5em}
% \begin{itemize}
%     \itemsep-0.25em 
%     % \item Add \lora~ layer to the aligned model for fine-tuning.
%     \item Feed harmful prompts and benign prompts into the aligned model and obtain the harmful direction $d_{h}$ and the benign direction $d_{b}$, respectively. 
%     \item Minimizes the harmful direction while keeping the benign direction by fine-tuning the layers before $L_d$.
% \end{itemize}

  

% Fine Tuning: We optimize the model parameters with
% QLoRA. The fine-tuning under all settings is run for one
% epoch, and the parameters are quantized to 4 bits. As suggested in, we set the rank and alpha of QLoRA to 8 and 16. We also set the learning rate to 2e−5 and the batch size to 96
%\yk{working on the following}
%\noindent\textbf{Results:} \autoref{tab:broken_direction}

%the harmful and aligned direction determines the LLM's alignment. In other words, if the hidden state of a prompt lies in the harmful direction, it will be rejected, otherwise, it will be answered. When applying this observation to the alignment broken phenomenon on fine-tuned LLM, we assume fine-tuning aligned LLM on harmful data shifts its harmful direction away from the initial harmful direction so that the harmful prompts will be answered. Therefore, we propose an approach to bring back the harmful direction of the fine-tuned LLM. 
 % Since the alignment can be undermined by pushing the harmful direction toward the aligned direction as demonstrated in \S\ref{subsec:method:insight}, we are wondering whether we can recover the alignment of the fine-tuned LLM by bringing back its harmful direction. 
 % of the LLM $\mathcal{M}_f$
 
%As shown in \autoref{fig:framework}, the alignment of the LLM $\mathcal{M}_f$, fine-tuned on $\mathcal{M}_a$, is sabotaged. To recover its alignment, we push its harmful direction toward the initial harmful direction of $\mathcal{M}_a$. To achieve this, we iteratively reset the partial parameters of the fine-tuned LLM $\mathcal{M}_f$ to the parameters of the aligned LLM $\mathcal{M}_a$ by the following steps. The details can be found in \autoref{alg:ggd}.


% we recover the alignment of the LLM $\mathcal{M}_f$, fine-tuned on $\mathcal{M}_a$, by aligning its harmful direction to that of $\mathcal{M}_a$.
% In algorithm \ref{alg:ggd}, we aim to recover the alignment of a fine-tuned LLM, denoted as $\mathcal{M}_f$, by aligning its harmful direction with the corresponding direction in the aligned LLM, $\mathcal{M}_a$, at a designated hidden layer $L_d$. This process involves resetting partial parameters of the fine-tuned LLM $\mathcal{M}_f$ to the parameters of the aligned LLM $\mathcal{M}_a$. To achieve this, we formulate the problem as a discrete optimization task and employ a gradient descent algorithm augmented with a greedy strategy. The algorithm comprises three main steps to accomplish this objective seamlessly. The first two steps are shown in \ref{fig:framework}. 

==> tables/parameters.tex <==
\begin{table}[!t]
        \scriptsize
	\centering
	\caption{Parameters used in fine-tuning reference models and local suspect models. \label{tab:parameters}}
	%\vspace{-0.75em}
	\begin{tabular}{l|l|l|l}
		\toprule
		\multirow{2}{*}{\textbf{Description}} & \multirow{2}{*}{\textbf{Parameter}} & \multicolumn{2}{c}{\textbf{Value}}\\
        & & R & M \\
        \midrule
	Rank of LoRA matrices & r & 8 & 8\\
		\midrule
		LoRA scaling factor &  lora\_alpha & 32 & 32\\
		\midrule
		Dropout probability for LoRA layers &  lora\_dropout & 0.05 & 0.05\\
        \midrule
        Bias type for LoRA & bias & none & none\\
        \midrule
        optimizer & optim & paged\_adamw\_8bit & paged\_adamw\_8bit \\
        \midrule
        learning rate & learning\_rate & $1 \times 10^{-4}$ & $1 \times 10^{-4}$ \\
        \midrule
        training batch size & 8 & 8 & 8 \\
        \midrule
        training epoch & num\_train\_epochs & 3 & 3 \\
        \midrule
        QLORA target modules & target\_modules & all linear & all linear \\
		\bottomrule
	\end{tabular}%
	%\vspace{-0.75em}
\end{table}%

==> tables/reference_architecture.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.2}
\footnotesize
\caption{Impact of architectural diversity of reference models on dataset inference. ``HF'' refers to Hugging Face.  A value ``x/y'' indicates that ``x'' out of ``y'' members/non-members are correctly identified. \label{tab:eval:ref_architecture}}
\setlength\tabcolsep{2.5pt}
\begin{tabular}{l|c|c|c|c|c}
\toprule
& \textbf{\# of Arch}                          & \textbf{Databricks} & \textbf{Alpaca} & \textbf{Slimorca} & \textbf{Openhermes} \\
\toprule
 \multirow{3}{*}{Local Members}     & 1     &  9/10          &  9/10      &  7/10        &  8/10        \\
 
 \cline{2-6}
 & 3                   &  10/10          &  10/10      &  9/10        &  9/10        \\
\cline{2-6}
 & 5                   &  10/10          &  10/10      &  10/10        &  10/10        \\
\cline{1-6}
 \multirow{3}{*}{HF Members} & 1      &   6/10         &  7/10      &  5/10        &  7/10        \\
 \cline{2-6}                         
  & 3               &  10/10          &  9/10      &  7/10        &  8/10        \\
  \cline{2-6}
 & 5                    &  10/10          &  10/10      &  10/10        &  10/10         \\
\cline{1-6}                         
 \multirow{3}{*}{HF Non-members}   & 1          &  20/20          &  20/20         &   20/20          &    20/20         \\
 \cline{2-6}
 & 3                 &  20/20          &  20/20         &   20/20          &    20/20          \\
 \cline{2-6}
 & 5                &  20/20          &  20/20         &   20/20          &    20/20          \\
\cline{1-6}                           
 \multirow{3}{*}{Precision (\%)}  & 1          &    100.0        &  100.0       &  100.0         & 100.0      \\

  \cline{2-6}
 & 3           &    100.0        &  100.0       &  100.0         & 100.0         \\
 \cline{2-6}
 & 5           &    100.0        &  100.0       &  100.0         & 100.0        \\
\cline{1-6}
 \multirow{3}{*}{Recall (\%)} & 1           &  75.0        &  80.0       &  60.0         & 75.0        \\
 \cline{2-6}                        
  & 3           &    100.0        &  95.0       &  80.0         & 85.0        \\
  \cline{2-6}
 & 5            &    100.0        &  100.0       &  100.0         & 100.0          \\
\cline{1-6}                        
 \multirow{3}{*}{F1 (\%)}    & 1               &   85.7         &   88.9     &   75.0       &   85.7        \\
 \cline{2-6}
  & 3           &    100.0        &  97.4       &  88.9         & 91.9          \\
  \cline{2-6}
 & 5           &    100.0        &  100.0       &  100.0         & 100.0         \\
\bottomrule                                     
\end{tabular}
\end{table}

==> tables/reference_number.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.36}
\footnotesize
\caption{Verification results of $\mathcal{M}$ with different number of reference models. Setting I and II are illustrated in \ref{sec:reference_models}. \label{tab:eval:ref_number}}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{l|c|c|c|c|c}
\cline{1-6}
& Setting                          & Databricks & Alpaca & Slimorca & Openhermes \\
\cline{1-6}
 \multirow{2}{*}{Non-members (1)}     & I       & 5/5           & 5/5       &  5/5        & 5/5           \\
 
 \cline{2-6}
 & II                   & 5/5          & 5/5       & 5/5         &  5/5          \\
\cline{1-6}
 \multirow{2}{*}{Non-members (2)} & I      & 20/20           & 20/20       & 18/20         &  17/20          \\
 \cline{2-6}                         
  & II              & 20/20           & 20/20       & 19/20         &  18/20        \\                          
\cline{1-6}                                    
\end{tabular}
\end{table}

==> tables/reference_number_and_architecture.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.36}
\footnotesize
\caption{Verification results of $\mathcal{M}$ with different architectures of reference models under IID\label{tab:eval:ref_number_arch}}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{l|c|c|c|c|c}
\cline{1-6}
& Setting                          & Databricks & Alpaca & Slimorca & Openhermes \\
\cline{1-6}
 \multirow{2}{*}{Non-members (1)}     & I       & 5/5           & 5/5       &  5/5        & 5/5           \\
 
 \cline{2-6}
 & II                   & 5/5          & 5/5       & 5/5         &  5/5          \\
\cline{1-6}
 \multirow{2}{*}{Non-members (2)} & I      & 20/20           & 20/20       & 19/20         &  18/20          \\
 \cline{2-6}                         
  & II              & 20/20           & 20/20       & 20/20         &  18/20        \\                          
\cline{1-6}                                    
\end{tabular}
\end{table}

==> tables/remove_samples.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.36}
\scriptsize
\caption{Verification results of $\mathcal{M}$ after removing tainted samples. \label{tab:eval:remove_samples}}
\resizebox{\columnwidth}{!}
{\begin{tabular}{c|l|c|c|c|c}
\hline
     &                     & Databricks & Alpaca & Slimorca & Openhermes \\
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{Epoch I}} & Local Members            & 9/10           & 10/10       &  10/10        & 10/10           \\
\cline{2-6}
 & HF Non-members  & 20/20           & 20/20       & 20/20         &  20/20          \\
\cline{2-6}                         
 & Precision (\%)                &   90.0         &   100.0      &   100.0        &   100.0         \\
\cline{2-6}                         
 & Recall (\%)                   &  100.0          &  100.0      &    100.0      &    100.0        \\
\cline{2-6}
& F1 (\%)                   &  94.7          &   100.0     &   100.0       &  100.0          \\
\hline        
\multirow{5}{*}{\rotatebox[origin=c]{90}{Epoch II}} & Local Members            & 8/10           & 9/10       &  9/10        & 8/10           \\
\cline{2-6}
 & HF Non-members  & 20/20           & 20/20       & 20/20         &  20/20          \\
\cline{2-6}                         
 & Precision (\%)                &   80.0         & 90.0        &   90.0        &  80.0          \\
\cline{2-6}                         
 & Recall (\%)                   &   100.0         & 100.0       &  100.0        &  100.0          \\
\cline{2-6}
& F1 (\%)                   &   88.9         &  94.7      &   94.7       &   88.9         \\
\hline      
\multirow{5}{*}{\rotatebox[origin=c]{90}{Epoch III}} & Local Members            & 6/10           & 8/10       &  7/10        & 7/10           \\
\cline{2-6}
 & HF Non-members  & 20/20           & 20/20       & 20/20         &  20/20          \\
\cline{2-6}                         
 & Precision (\%)                &   60.0         &  80.0       &  70.0         &  70.0          \\
\cline{2-6}                         
 & Recall (\%)                   &   100.0         &  100.0      &  100.0        &  100.0          \\
\cline{2-6}
& F1 (\%)                   &   75.0         &  88.9      &  82.4        &     82.4       \\
\hline      
\end{tabular}
}
\end{table}

==> tables/remove_tainted_samples.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.36}
\footnotesize
\caption{Verification results of local $\mathcal{M}$ trained on $\mathcal{D}$ excluding tainted samples. \label{tab:eval:remove}}
\setlength\tabcolsep{9.5pt}
\begin{tabular}{l|c|c|c|c}
\cline{1-5}
                          & Databricks & Alpaca & Slimorca & Openhermes \\
\cline{1-5}
 Members            &   10/10         &   10/10     &   10/10       &    10/10        \\
\cline{1-5}
\end{tabular}
\end{table}

==> tables/rephrase.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.36}
\footnotesize
\caption{Verification results of $\mathcal{M}$ with tainted samples under rephrasing. \label{tab:eval:rephrase}}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{l|c|c|c|c}
\cline{1-5}
                          & Databricks & Alpaca & Slimorca & Openhermes \\
\cline{1-5}
 Local Members            & 10/10           & 10/10       &  10/10        & 10/10           \\
\cline{1-5}
 Hugging Face Members & 10/10           & 10/10       & 10/10         &  10/10          \\
\cline{1-5}
 Hugging Face Non-members & 20/20           & 20/20       & 20/20         &  20/20          \\
\cline{1-5}                        
 Precision (\%)                &  100.0          & 100.0       &  100.0        & 100.0        \\
\cline{1-5}                          
 Recall (\%)                   &  100.0          & 100.0       &  100.0        & 100.0           \\
\cline{1-5}
F1 (\%)                   &  100.0          & 100.0       &  100.0        & 100.0           \\
\cline{1-5}                                             
\end{tabular}
\end{table}

==> tables/subset.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.36}
\footnotesize
\caption{Verification results of local $\mathcal{M}$ trained on subsets of $\mathcal{D}$. "OL"
refers to overlapping and "NOL" refers to non-overlapping.\label{tab:eval:subset}}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l|c|c|c|c|c}
\cline{1-6}
                 &         Setting & Databricks & Alpaca & Slimorca & Openhermes \\
\cline{1-6}
  \multirow{2}{*}{OL Members}            & I    &   5/5         &   5/5     &   5/5       &    5/5        \\
\cline{2-6}
& II    &   5/5         &   5/5     &   4/5       &    3/5        \\
\cline{1-6}
  \multirow{2}{*}{NOL Members}       & I     &    10/10        &  10/10      &   9/10       &   9/10         \\
  \cline{2-6}
  & II  &    9/10        &  9/10      &   7/10       &   8/10        \\
\cline{1-6}
\end{tabular}
\end{table}

==> tables/temperature.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.36}
\footnotesize
\caption{Verification results of $\mathcal{M}$ with different values of the temperature. Setting I, II and III are illustrated in \ref{sec:temperature}.  \label{tab:eval:temperature}}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{l|c|c|c|c|c}
\cline{1-6}
& Setting                          & Databricks & Alpaca & Slimorca & Openhermes \\
\cline{1-6}
 \multirow{3}{*}{Local Members}     & I       &  10/10          &  10/10      &  10/10        &   10/10         \\
 
 \cline{2-6}
 & II                    &  10/10          &  10/10      &  10/10        &   10/10          \\
\cline{2-6}
 & III                    &  10/10          &  10/10      &  10/10        &   10/10          \\
\cline{1-6}
 \multirow{3}{*}{Hugging Face Members} & I       &  10/10          &  10/10      &  10/10        &   10/10          \\
 \cline{2-6}                         
  & II               &  10/10          &  10/10      &  10/10        &   10/10        \\
  \cline{2-6}
 & III                    &  10/10          &  10/10      &  10/10        &   10/10          \\
\cline{1-6}                        
 \multirow{3}{*}{Hugging Face Non-members}   & I                &  20/20          &  20/20        &   20/20        &  20/20          \\
 \cline{2-6}
 & II                 &  20/20          &  20/20        &   20/20        &  20/20           \\
 \cline{2-6}
 & III                   &  20/20          &  20/20        &   20/20        &  20/20          \\
\cline{1-6}                          
 \multirow{3}{*}{Precision (\%)}  & I          &  100.0          &  100.0         &  100.0          &  100.0            \\
 
  \cline{2-6}
 & II           &  100.0          &  100.0         &  100.0          &  100.0         \\
 \cline{2-6}
 & III                   &  100.0          &  100.0         &  100.0          &  100.0        \\
\cline{1-6}
 \multirow{3}{*}{Recall (\%)} & I           &  100.0          &  100.0         &  100.0          &  100.0        \\
 \cline{2-6}                        
  & II             &  100.0          &  100.0         &  100.0          &  100.0     \\
  \cline{2-6}
 & III                   &  100.0          &  100.0         &  100.0          &  100.0       \\
\cline{1-6}                        
 \multirow{3}{*}{F1 (\%)}    & I               &  100.0          &  100.0         &  100.0          &  100.0           \\
 \cline{2-6}
  & II                &  100.0          &  100.0         &  100.0          &  100.0          \\
  \cline{2-6}
 & III                   &  100.0          &  100.0         &  100.0          &  100.0       \\
\cline{1-6}                                  
\end{tabular}
\end{table}
